Magnetic-Reconnection-Heated Corona Model: Implication of Hybrid Electrons for Hard X-ray Emission of Luminous Active Galactic Nuclei

It is widely accepted that X-ray emission in luminous active galactic nuclei (AGNs) originates from hot corona. To prevent the corona from over-cooling by strong X-ray emission, steady heating to the corona is essential, for which the most promising mechanisms is the magnetic reconnection. Detailed studies of the coupled disc and corona, in the frame of magnetic field transferring accretion-released energy from the disc to the corona, reveal that the thermal electrons can only produce X-ray spectrum with $\Gamma_{\rm 2-10\,keV}>2.1$, which is an inevitable consequence of the radiative coupling of the thermal corona and disc. In the present work, we develop the magnetic-reconnection-heated corona model by taking into account the potential non-thermal electrons accelerated in the magnetic reconnection process, in addition to the thermal electrons. We show that the features of the structure and spectrum of the coupled disc and corona can be affected by the fraction of magnetic energy allocated to thermal electrons. Furthermore, we investigate the effects of the power-law index and energy range of non-thermal electrons and the magnetic field on the spectrum. It is found that the X-ray spectrum from the Comptonization of the hybrid electrons can be flatter than that from thermal electrons only, in agreement with observations. By comparing with the observed hard X-ray data, we suggest that a large fraction ($>40\%$) of the magnetic energy be allocated to the non-thermal electrons in the luminous and flat X-ray spectrum AGNs.

==> README <==
This is the README for the mweights package, version
2020-01-23.

Many font families available for use with LaTeX have multiple
weights, especially when originally aimed at use on the web. For
example, Linux Libertine has both bold and semibold; Cabin, a
sans-serif family, has four weights (regular, medium, semibold,
bold); SourceCodePro, a monospaced family, has seven weights.

Traditionally the type1-oriented support packages for such fonts
re-define the standard \mddefault or \bfdefault macros. But this can
create difficulties if the weight desired for one font family isn't
available for another font family, or if it differs from the weight
desired for another font family. For example, there is no medium
weight font for Linux Libertine so that setting \mddefault to mb for
use with Cabin will be problematic for Libertine. And \bfdefault
cannot be both sb for use with Cabin and b for use with Libertine,
or vice versa.

This package provides a solution to these difficulties. The basic
idea (due to Michael Sharpe) is that font packages should *not*
re-define \mddefault or \bfdefault; instead they should define as
many of the following macros as is appropriate:

\mdseries@rm
\mdseries@sf
\mdseries@tt

\bfseries@rm
\bfseries@sf
\bfseries@tt

For example, 

\def\mdseries@sf{mb}
\def\bfseries@sf{b}

would be appropriate definitions for using a sans font such as Cabin 
with medium and bold, and

\def\bfseries@rm{sb}

would be appropriate for using a Roman font such as Libertine
with semibold. These macros should always be fully expanded; if
necessary, \edef should be used.

The package re-defines standard selection commands for series
(\mdseries and \bfseries) and family (\rmfamily, \sffamily,
\ttfamily) to use the macros. It should be a RequiredPackage (for
type1 font use only) in any such font package.

This package need not be used with LaTeX releases after
2020-02-02 which will incorporate mweights functionality
into the LaTeX kernel; the mweights package itself will
actually not be loaded by the kernel.

The package is licensed under the terms of the LaTeX Project
Public License. The maintainer is Bob Tennent (rdt at
cs.queensu.ca).

